UtilCache: Effectively and Practicably Reducing Link Cost in Information-Centric Network

Minimizing total link cost in Information-Centric Network (ICN) by optimizing content placement is challenging in both effectiveness and practicality. To attain better performance, upstream link cost caused by a cache miss should be considered in addition to content popularity. To make it more practicable, a content placement strategy is supposed to be distributed, adaptive, with low coordination overhead as well as low computational complexity. In this paper, we present such a content placement strategy, UtilCache, that is both effective and practicable. UtilCache is compatible with any cache replacement policy. When the cache replacement policy tends to maintain popular contents, UtilCache attains low link cost. In terms of practicality, UtilCache introduces little coordination overhead because of piggybacked collaborative messages, and its computational complexity depends mainly on content replacement policy, which means it can be O(1) when working with LRU. Evaluations prove the effectiveness of UtilCache, as it saves nearly 40% link cost more than current ICN design.

==> sections/algorithm.tex <==
\section{UtilCache: Distributed algorithm}
\label{algorithm}
% 从上节可以知道，在某个请求分布下，只要找到……的前C个就可以了，在实际应用场景中如何找呢？
% 1. 一定需要记录额外信息：LRU等方式存在admission问题，【为什么admission一定要额外信息？】
% 2. 记录信息开销大
% 本节介绍了如何解决这些问题
From \eqref{pd} we understand that, suppose the cache size is $B$, the best choice for each router is to cache contents with top $B$ highest caching utility. The problem is, however, how to realize it, i.e.\ to figure out these contents, in a distributed, adaptive manner, which is more scalable and practical. In this section, we present a caching strategy, \textbf{UtilCache}, that meets the demand. 

\subsection{Caching Strategy}
% 具体操作
% 特点：1. 额外考虑了d
%     2. 有admission
The proceeding of UtilCache comprises three components: (1) Utility Estimation; (2) Cache Polices, where utility estimation is of paramount importance because the veracity of it has a direct impact on whether a content blocked out (admitted in) is wronged (an impostor). 

We first cast a look at general framwork of UtilCahce (Fig.~\ref{ucache}), leaving the detailed elaboration of utility estimation in Sec~\ref{UE}.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.45\textwidth]{pic/1.png}\\
\caption{UtilCache Framework}
\label{ucache}
\end{figure}

Firstly and Fundamentally, for any given content, its caching utility is estimated. Whenever a new content arrives at a router with full cache, cache policy prioritizes contents (including the new content) by caching utility and chooses a potential victim with lowest caching utility. The new content will be blocked out if it is exactly the victim, or else it will take the place of the victim. It is similar to LFU with the only difference lies in that LFU prioritizes contents by frequency.
All in all, UtilCache makes a two-pronged effort in both cache admission and replacement to retain the high-utility contents, blocking and evicting the low-utility ones.

\subsubsection{Utility Estimation}
\label{UE}
Utility estimation essentially comprises the estimation of content popularity and upstream link cost:

\textbf{Popularity Estimation. } At each router, there is a popularity counter for each content that counts up the number of requests for this content in a given time interval $T$. When next interval comes, popularity estimation is updated to a new value from the counters and the counters are reset.
%Popularity of each content can be obtained at each node by counting and recording how much content requests (from both local clients and other routers) arrives in a certain time interval (a.k.a. unit time).

\textbf{Upstream Link Cost Estimation. } Each node is supposed to maintain the estimation of \emph{average} upstream link cost. It occurs to us intuitively that the information of upstream link cost can be piggybacked by the returned data packets. We add a field for \emph{Upstream Link Cost} estimation in the data packet, named ULC. If a request from $s$ is satisfied at $t$, ULC of the data packet generated at $t$ is inited to 0. Whenever it is transferred from $j$ to $i$ via link $(i,j)$, ULC in it is added by $w_{ji}$. Intermediate nodes can update their estimation by sniffing the ULC field of the arriving data packets. To emphasize the importance of fresh statistics, the average upstream link cost is calculated as a moving average:
$$\bar{d}^c_i=\alpha d^c_i+(1-\alpha)\bar{d}^c_i$$

\subsection {Variants to Meet Practical Demands}
The physical meaning of \eqref{pd} makes it more free to adjust the cache scheme to meet practical demands, with the only rationale to keep in mind: \emph{cache those with higher caching utility}.
 
\subsubsection{Space Reduction}
In some cases, logging all the raw utility information, especially the popularity information, is too space-inefficient, for which we want to reduce the space consumption \emph{without much loss of performance}. 
%In U-Cache, therefore, we use a sliding window to screen out the recently requested content and thus only their records of \emph{both popularity and mean upstream distance} are maintained, which depresses the consumed space of statistics while keeps it fresh as well.

A simple solution is to set a maximal threshold as $W$ to limit the bits of each counter. Upon updating a counter of popularity (upstream link cost) estimation, if the value of this counter exceeds $W$, values of all the popularity (link cost) counters at this router will be divided by a constant factor $e$ (e.g.\ $e=2$). As a result, the space for estimating popularity (upstream link cost) is controlled within a limit.

Another advanced solution is to use space-compact approximate counting architectures (e.g.\ Spectral Bloom Filter\cite{sbf}, Count Min Sketch\cite{cm-sketch}). In this paper, we use \emph{Counting Bloom Filter} (CBF)\cite{cbf} to count the popularity of each content. CBF is a bloom filter whose entries are counters rather than a single binary bit. More detailedly, a CBF consists of an array of counters and $k$ hash functions each mapping the content to a counter. Thus for a given content, there are $k$ corresponding counters which are all added by one when the counting value of this content needs an increment. The minimal value of these counters is the estimated counting value for the content. CBF answers the counting queries with appealing space and time complexity and yet a tunable low probability of false positives.

\subsubsection{More Adaptive}
Sometimes the popularity law and request arrival rate vary frequently, which is common in real request traces. In these cases, estimating utility by the history statistics is no longer applicable and thus a more adaptive cache scheme is needed.









==> sections/conclusion.tex <==
\section{conclusion}
\label{conclusion}

This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings. of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.This paper provides a sample of a \LaTeX\ document which conforms,
somewhat loosely, to the formatting guidelines for
ACM SIG Proceedings.

==> sections/evaluation.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.4\textwidth]{pic/theory.pdf}\\
\caption{Numerical Evaluations for approximate models}
\label{numevares}
\end{figure}

\section{Performance Evaluation}
\label{eva}

\begin{figure*}[htbp]
\centering
\subfigure[Zipf Exponent $\alpha \in \{0.6,0.8,1.0,1.2,1.4\}$ and fixed Cache to population ratio $C=0.01$
\label{fixedtopo:0}]{
\centering
\includegraphics[width=0.9\textwidth]{pic/fixedtopo-0.pdf}
}
\subfigure[Cache to population ratio $C\in \{0.002,0.005,0.01,0.03,0.05\}$ and fixed Zipf Exponent $\alpha=1.0$
\label{fixedtopo:1}]{
\centering
\includegraphics[width=0.9\textwidth]{pic/fixedtopo-1.pdf}
}
\caption{Performance of each cache schemes with fixed network topology.}
\label{fixedtopores}
\end{figure*}

In this section, we first do numerical evaluations to examine solution of two approximate model: $LCM-L$ and Pipage-Rounding (PR). Results shows that they attain very close performance in most situations, which indicates our approximate model yields certain optimality guarantees in usual cases. Then we evaluate the performance of several cache schemes, comparing our distributed algorithm with other state-of-the-arts. Simulation results validate its efficacy and low overhead.

\begin{table}
  \caption{Network Topologies}
  \label{simtopo}
  \begin{tabular}{{r}|*{3}{c}}
    \toprule
    & Nodes & Edges & Max Degree\\
    \midrule
    GEANT & 51 & 64 & 7\\
    TOPO50 & 53 & 74 & 10 \\
    TOPO200 & 203 & 364 & 14\\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Experimental Setup}
In our evaluations, we set the link cost \emph{equally to 1}, which represents a single hop. Thus, the Link Cost Minimization problem turns to a subproblem \emph{Hop Count Minimization} problem.

\textbf{Networks. }Simulations involve three topologies: GEANT \cite{geant}, TOPO50 and TOPO200. GEANT is a core network interconnecting several European research institutes and universities, while TOPO50 and TOPO200 are two scale-free topologies generated with aSHIIP \cite{ashiip} following a hierarchical Barabasi-Albert model (m = 2). Details are in Tab.~\ref{simtopo}.

\textbf{Workloads. }We suppose that there are a given number of contents in the whole network whose popularities follow the Zipf law. Content requests are generated with a give arrival rate. We use Icarus \cite{icarus}, a discrete-event simulator offering flow-level simulations in our experiments. The content are equal-sized as 1, and the arrival process of requests is assumed to be Poisson process.

\textbf{Parameters. }We mainly consider the effect of three parameters: \emph{Zipf exponent $\alpha$}, \emph{cache to population ratio} and \emph{topology}. Zipf exponent $\alpha$ indicates the skewness of popularity distribution. When $\alpha$ increases, the popular items become further popular and unpopular ones less. Cache to population ratio, introduced in \cite{hashrouting}, shows the proportion of total cache size to total content size.

\textbf{Performance Metrics. }We evaluate the performance of each cache scheme with three metrics: \emph{Total Link Cost}, \emph{Coordination Overhead} and \emph{Server Load}. Total link cost is measured by the total hop count for all the requests, while coordination overhead by the number of packets propagated to deliver informations. Server load refers to the server hit ratio, i.e.\ the proportion of content requests satisfied at designated source.

\begin{figure*}[htbp]
\centering
\subfigure[TOPO50 with $\alpha=1.0$ and $C=0.01$
\label{changetopo:0}]{
\centering
\includegraphics[width=0.9\textwidth]{pic/changetopo-0.pdf}
}
\subfigure[TOPO200 with $\alpha=1.0$ and $C=0.01$
\label{changetopo:1}]{
\centering
\includegraphics[width=0.9\textwidth]{pic/changetopo-1.pdf}
}
\caption{Performance on topologies of different scales.}
\label{changetopores}
\end{figure*}


\subsection{Comparison Between Approximate Models}
$LCM-L$ and Pipage-Rounding (PR) in \cite{26} can be regarded as two models giving an approximate solution to $LCM-G$ in a centralized way. Ioannidis et al.\ proves that Pipage-Rounding gives a solution with $1-1/e$ factor from the optimal and thus we are curious about the performance of $LCM-L$ and do numerical evaluations.

The number of contents are set to be 100. We tune the Zipf exponent $\alpha$ from 0.6 to 1.4, and cache to population ratio from 0.3 to 0.7 (a little high because of few contents), respectively. The solutions of $LCM-L$ (Algorithm~\ref{centralizedalgo}) and Pipage-Rounding (\cite{26}) are calculated in different scenarios, and finally we have the total link cost $G(\mathbf{X})$ calculated by the given solutions.

Fig.~\ref{numevares} shows the results of numerical evaluations. We speculate on the performance of $LCM-G$'s optimal solution (i.e.\ the shadow in each graph), according to the optimality guarantees of Pipage-Rounding. We know that our approximate model $LCM-L$ attains similar or even higher performance compared with Pipage-Rounding when network configuration changes, which means $LCM-L$ have certain optimality guarantees as well, in most cases.

\subsection{Link Cost Saving}
\label{simlcs}
We evaluate the performance of distributed caching schemes, comparing UtilCahce with other state-of-the-arts: Leave Copy Everywhere (LCE) \cite{metaalgo}, ProbCache \cite{probcache}, Projected Gradient Ascent (PGA) \cite{26} and UtilCache. LCE is the simple cache scheme applied in ICN mostly. ProbCache is a cache scheme with probabilistic cache admission policy, the probability to admit a content decided empirically. PGA, however, is a cache scheme designed based on a theoretical model with optimality guarantees. For LCE, ProbCache and PGA, the cache replacement policy for each single cache is LRU.

There are $3\times 10^5$ contents in the whole network, and content requests are generated with a rate of 12 requests per second. We use $3\times 10^5$ requests which is not logged to warm up the caches, and another $6\times 10^5$ requests to generate results. 

Experiments in this section focus on the performance in regard to link cost saving. Topology is fixed to be TOPO50, while Zipf exponent $\alpha$ and cache to population $C$ varies in $[0.6, 1.4]$ and $[0.002, 0.05]$, respectively.

Results in Fig.~\ref{fixedtopores} shows UtilCache performs best among the four. 
Compared with PGA, UtilCache yields lower link cost, which validate the efficacy of our approximate model $LCM-L$. UtilCache introduces less coordination overhead as well, because information is piggybacked in data packet and it will be returned once the request is satisfied. In PGA, however, information should be carried in additional packets as they sometimes need to be disseminated further to source after a cache hit. Since the average hop count for a request is less in UtilCache, request/data packets in the network decrease accordingly, for which UtilCache narrowly edges out ProbCache and LCE. Outperformance of UtilCache over ProbCache manifests the benefit of theoretical analysis as well.
In addition, UtilCache makes better utilization of caches by caching less junk content, thus leading to more cache hit and less server load.

\subsection{Scalability}
To test the scalability, we run experiments on topologies of different scale: \emph{TOPO50} and \emph{TOPO200}. Zipf exponent $\alpha$ and cache to population $C$ are fixed to be 1.0 and 0.01 respectively. Without loss of generality, designated sources are randomly assigned at the beginning of each run, and for each topology we do 100 runs in case of contingency. Other configurations are exactly the same as in Sec.~\ref{simlcs}.

Results are depicted in Fig.~\ref{changetopores}. When the topology becomes larger (with more nodes, more links, and more caches), UtilCache remains to have lowest link cost and server load. It should be noted that the increase of coordination overhead is rather inconspicuous for UtilCache, which contributes to the high scalability of UtilCache. ProbCache and LCE are scalable as well, yet they yields more link cost and server load. For PGA, however, despite its efficacy, the high overhead limits its scalability and thus the practicality. 


==> sections/global.tex <==
\section{LCM-G: the Global Model}
\label{globalmodel}

The global model is built under a global view of network state, whose optimal solution gives the upper bound of cache performance. In this section, we formulate the \emph{Link Cost Minimization (LCM)} problems based on the aforementioned ICN features.

% 全局模型能得到在分布固定的某个瞬间的最优决策，提供了性能的上界。本节结合ICN实际特点进行模拟，最后提出全局模型

\subsection{Assumptions}

Before introducing the global model, we make several reasonable assumptions:

% 1. IRM
%     为什么？【实验分布的locality和收敛速度和时间间隔的关系】
%     本文里的popularity指的啥

\textbf{Independent Reference Model. } Requested contents fall into a fixed catalogue of $|\mathbf{C}|=m$ objects following a stationary popularity law $q(\cdot)$, a.k.a.\ Independent Reference Model (IRM) \cite{IRM1}. That is, for each content $c\in \mathbf{C}$, a request is for $c$ with constant probability $q(c)$. Suppose the total request rate is $\lambda$. The request rate for content $c$ is evidently $\lambda q(c)$. We refer to popularity as \emph{per content request rate} $p(\cdot) = \lambda q(\cdot)$ hereafter.
IRM ignores the \emph{temporal locality}, a significant feature in real content request traces, that embodies the temporal correlations between requests. Traverso et al.\ \cite{temporal} have presented a Shot Noise Model (SNM) to capture the dynamics of content popularity. Analytical models under SNM, however, show to be challenging \cite{snmdifficult}. Therefore, we still consider the IRM in our global model.

%in spite of which the distributed adaptive algorithm (Sec.\ \ref{algorithm}) derived from it is validated to be efficient in evaluations using real request traces (Sec.\ \ref{eva}).

% 等大小：chunk、MCU等机制
\textbf{Equal-sized Contents. } Every content in the network has unified size. Since the derivation is similar without this assumption, we still keep it for simplicity considerations.

% 2. 忽略PIT【引用前作】
\textbf{No Request Aggregation. } We suppose there exists no content request aggregation mechanism such as the well-known Pending Interest Table (PIT) in Name-Data Network (NDN)\cite{ndn}, as J.J. Garcia-Luna-Aceves et al.\ \cite{ccnramp,pit1,pit2} have expounded PIT does not deliver substantial benefits but is likely to cause problems counter-productively.

% 对称性
\textbf{Symmetric Path. } Content request and the corresponding data packet traverse the same path, which is a common assumption in the context of ICN, similarly to \cite{probcache,intraas,26,joint1}.

\textbf{Instantaneous Data Return. } Data packets are supposed to be returned instantaneously, or at least in a small delay negligible compared with the request arrival process. This assumption results in the equal arrival rate for both requests and contents.

\textbf{Negligible Link Cost of Requests. } We calculate the total link cost considering only what is caused by data packets, because content requests are much smaller than data packets and thus link cost (latency, bandwidth etc.) caused by them is negligible.

\subsection{Problem Formulation}

\begin{table}
  \caption{Notations}
  \label{simtopo}
  \begin{tabular}{cl}
    \toprule
    $\mathbf{G}=\langle\mathbf{N}, \mathbf{E}\rangle$ & Network topologies\\
    $B_i$ & Cache size for router $i$\\
    $\pi^c_{ij}$ & Probability to forward request for $c$ from $i$ to $j$ \\
    $x^c_i$ & $x^c_i=1$ means router $i$ caches content $c$\\
    $p^c_i$ & Popularity of $c$ at $i$\\
    $f^c_{ij}$ & Request transferring rate for content $c$ from $i$ to $j$\\
    $w_{ij}$ & Cost caused by transferring a packet from $i$ to $j$\\
    \bottomrule
  \end{tabular}
\end{table}

% 1. 网络->图：只把cache相连的图
The whole cache network (Feature \ref{feature:1}) can be represented as an undirected graph $\mathbf{G}=\langle\mathbf{N}, \mathbf{E}\rangle$, where $\mathbf{N}=\{1,...,n\} $ is a set of nodes as the caches and each edge $(i,j)$ in the edge set $\mathbf{E}$ indicates packets can be transmitted bidirectionally between node $i$ and $j$.
For each node $i\in \mathbf{N}$, its cache capacity is $B_i$.

% 2. 路由路径：1. 每个内容不同，分别是一个DAG，且为概率
Missed requests for $c$ at node $i$ are forwarded to $j$ with probability $\pi^c_{ij}$. Thus $\{\pi^c_{ij}|i,j\in\mathbf{N}\}$ represents the different routing decision for each $c\in\mathbf{C}$ (Feature \ref{feature:4}), comprising the feasible routes to multiple designated sources in $\mathbf{S^c}$ (Feature \ref{feature:2}). Unsatisfied requests should not cease to be forwarded unless arriving at designated source, and consequently we have $\sum_{j\in\mathbf{N}}\pi^c_{ij}=1$ for all $i\in\mathbf{N}-\mathbf{S^c}$, and $\sum_{j\in\mathbf{N}}\pi^c_{ij}=0$ for all $i\in\mathbf{S^c}$. $\pi^c_{ij}$ is in $\{0,1\}$ in our previous work \cite{utilcache} as a single-path routing decision. In this paper, however, the constraint is relaxed to $[0,1]$ as there are multiple alternative next hops for a node to choose (Feature \ref{feature:3}).

% 3. cache策略：因为是二元的，所以是矩阵变量
Network cache decisions, \emph{the only independent variables} of our global model, are denoted by a matrix $\mathbf{X}=[x^c_i]_{i\in\mathbf{N},c\in\mathbf{C}}\in \{0,1\}^{|N|\times|C|}$. $x^c_i$ is binary indicating whether content $c$ is cached in node $i$ ($x^c_i=1$ if being cached).

% f{ijc}的定义：这条边的权重，在最简单的情况下，就是单位时间通过的请求数
We use $p^c_i$ to denote the popularity of content $c$ at router $i$, i.e.\ the arrival rate of requests for $c$ at $i$. In most networks (e.g.\ ISPs), routers (or nodes) are classified into edge routers and core routers, with only edge routers able to received content requests from users directly. Let $\mathbf{R}\in\mathbf{N}$ refer to the set of edge routers. In LCM problems, request arrival rate at edge routers is constant yet that at core routers is variable depending on cache decisions. Let $f^c_{ij}$ be the number of requests being transferred from $i$ to $j$ in unit time. 

%we suppose that, for generality, each node $i$ receives content request for $c$ at a rate of $l^c_i$. $l^c_i$ can be set to $0$ when $i$ is a so-called core router, which does not bring about significant differences in our analysis. We define $f^c_{ij}$ as the total request rate for content $c$ from node $i$ to $j$. 

In our formulation, transferring a packet from router $i$ to $j$ is supposed to be $w_{ij}$. Notice that $w_{ij}$ and $w_{ji}$ are not necessarily equal. Now we can formulate the Link Cost Minimization problem into a global model $LCM-G$:

\begin{alignat}{2}
\min\quad & G(\mathbf{X})=\sum_{i\in\mathbf{N}}\sum_{j\in\mathbf{N}}w_{ji}(\sum_{c\in\mathbf{C}}{f^c_{ij}})&{}& \label{GM:1}\\
\mbox{s.t.}\quad &B_i-\sum_{c\in\mathbf{C}}{x^c_i}\ge 0 &{}&,\forall i\in\mathbf{N}\label{GM:2}\\
&x_i^c\in\{0,1\}&{}&,\forall c\in\mathbf{C},\forall i\in\mathbf{N}\label{GM:3}\\
&f^c_{rj}=\pi^c_{rj}p^c_r(1-x^c_r)&{}&,\forall c\in\mathbf{C},\forall r\in\mathbf{R}, j\in\mathbf{N}\label{fij:1}\\
&f^c_{ij}=\pi^c_{ij}(\sum_{v\in \mathbf{N}}f^c_{vi})(1-x^c_i)&{}&,\forall c\in\mathbf{C},\forall i\in\mathbf{N}-\mathbf{R}, j\in\mathbf{N}\label{fij:2}
\end{alignat}

\eqref{GM:1} represents the total link cost per unit time for us to minimize. \eqref{GM:2} and \eqref{GM:3} are the capacity and integrality constraints, respectively. \eqref{fij:1} and \eqref{fij:2} shows the calculation of $f^c_{ij}$, from which we can know $p^c_i=\sum_{v\in \mathbf{N}}f^c_{vi}$ for $i\in\mathbf{N}-\mathbf{R}$.

We can run an offline, centralized algorithm based on $LCM-G$, gathering the network state and computing the optimal solution of it as the cache decisions. Despite feasibility, the algorithm gives the optimal content placement that attains the highest cache performance as an upper bound.

==> sections/local.tex <==
\section{LCM-L: the Local Model}
\label{localmodel}
% 1. 解全局问题NP-HARD
% 2. 实际场景中也难以做到
% 本节提出本地视角的近似手段，推导出一个在本地视角下，与全局模型等价的模型，并为下文的分布式算法做启发。

Running an offline algorithm in centralized way is impracticable due to the costly information dissemination and high computing complexity. Worse still, $LCM-G$ turns our to be NP-hard. 

In this section, we first introduce \emph{Local View}, an approximate hypothesis under which the only variables are local caching decisions. Then we derive a model equivalent to the global model under local view (named local model), paving the way for our distributed algorithm in Sec.~\ref{algorithm}.

\subsection{Local View}

% 是什么？
% 为什么？
% 1. 实际场景下单个cache不知道其它人存了什么。
%     有工作交换这些信息，但是（1）开销大（2）不及时
% 2. 既然这样，不如转化成A的状态与外界状态的互动问题

In most of the situations, it is rather difficult for a single router to know the cache state of others, let alone to decide it.

In some works \cite{2016scalable,muncc,wong}, cache summaries are exchanged between routers. Although space-efficient data structure (e.g.\ Bloom Filter\cite{bloomfilter}) is applied to depress the communication overhead, another vital drawback for this cache summary sharing method is the freshness and consistence of the information stored in each router because their algorithms depend on a large amount of external information. Since outdate records certainly bring about performance loss, 
"a large amount of outdate records" make things worse.

%For example, information recorded in router $A$ indicates the requested content is cached in router $B$, as a result of which $A$ forwards the content request to $B$ rather than the source server. However, the content in $B$ has been evicted before the redirected request arrives, due to the frequent cache replacement. In this case, the redirection is in vain but causes extra communication overhead.

%     cache状态变化速度（用车浩公式推导）    vs    传播速度    +    传播开销复杂度

Consequently, we come up with our approximate hypothesis, Local View:

\paragraph{Local View} Only local cache decisions are independent variables and other cache decisions remain constant. Specifically, for router $A$, the independent variable is $\mathbf{X_A}=\langle x^1_A,...,x^ m_A\rangle$, which is named \emph{A's View} as well.\\

The thinking in \emph{Local View Approximation} is similar to the "sub gradient" in \cite{26}. Both of them intend to reduce the scope of independent variables, yet Local View Approximation leads to more uncomplicated analysis results with specific physical meaning.

\subsection {Local Model}


\subsection{Optimal Solution for Local Model}
\label{utility}
% 最优解
$LCM-L$ is a simple integer linear programming problem. It is easy to know that its optimal solution is as follows:
\paragraph{Optimal Solution for $LCM-L$} Suppose $p^1_A\bar{d}^1_A>p^2_A\bar{d}^2_A>...p^m_A\bar{d}^m_A$, the optimal solution for $LCM-L$ is:
\begin{equation}
\label{pd}
X^c_A=\left\{\begin{matrix}
 1&, 1\leq c\leq B_A\\ 
 0&, \text{otherwise} 
\end{matrix}\right.
\end{equation}

We define $p^c_A\bar{d}^c_A$, the product of the popularity and average upstream link cost as the \emph{Caching Utility} of content $c$ at router $A$. The physical meaning of this optimal solution is evident: to keep those contents with highest caching utility in cache. Any content with low utility enters the cache may lead to suboptimal performance. This analytical result does prove the significance of cache admission. 
% 这个最优解说明别的内容都不应该进cache

==> sections/tmp.tex <==
\section{tmp}

$\mathcal{D}$:
\begin{subequations}
\begin{alignat}{2}
C(\mathbf{X})=\sum\limits_{c\in\mathbf{C}}p^c_A\bar{d}^c_A\cdot x^c_A &\label{LM:1}\\
  B_A-\sum_{c\in\mathbf{C}}{x^c_A}\ge 0 &{}&\label{LM:2}\\
&x_A^c\in\{0,1\}&{}&,\forall c\in\mathbf{C}\label{LM:3}
\end{alignat}
\end{subequations}

\begin{subequations}
\begin{alignat}{2}
\min\quad & C(\mathbf{X})=\sum\limits_{c\in\mathbf{C}}p^c_A\bar{d}^c_A\cdot x^c_A &{}& \label{LM:1}\\
\mbox{s.t.}\quad &B_A-\sum_{c\in\mathbf{C}}{x^c_A}\ge 0 &{}&\label{LM:2}\\
&x_A^c\in\{0,1\}&{}&,\forall c\in\mathbf{C}\label{LM:3}
\end{alignat}
\end{subequations}
